Studying the Practices of Deploying Machine Learning Projects on Docker

Docker is a containerization service that allows for convenient deployment of websites, databases, applications' APIs, and machine learning (ML) models with a few lines of code. Studies have recently explored the use of Docker for deploying general software projects with no specific focus on how Docker is used to deploy ML-based projects. In this study, we conducted an exploratory study to understand how Docker is being used to deploy ML-based projects. As the initial step, we examined the categories of ML-based projects that use Docker. We then examined why and how these projects use Docker, and the characteristics of the resulting Docker images. Our results indicate that six categories of ML-based projects use Docker for deployment, including ML Applications, MLOps/ AIOps, Toolkits, DL Frameworks, Models, and Documentation. We derived the taxonomy of 21 major categories representing the purposes of using Docker, including those specific to models such as model management tasks (e.g., testing, training). We then showed that ML engineers use Docker images mostly to help with the platform portability, such as transferring the software across the operating systems, runtimes such as GPU, and language constraints. However, we also found that more resources may be required to run the Docker images for building ML-based software projects due to the large number of files contained in the image layers with deeply nested directories. We hope to shed light on the emerging practices of deploying ML software projects using containers and highlight aspects that should be improved.

==> 05-discussion.tex <==
In Section~\ref{sec:results}, we presented our results answering our four proposed \textbf{RQs}. As our study's initial step, we categorised ML-based projects using Docker for deployment into six (6) categories, including ML Applications, MLOps/ AIOps, Tookits, DL Frameworks, Models, and Documentation. Indeed, the adoption of Docker  %\heng{docker vs. Docker} 
in these variety of ML software projects is not surprising given the numerous advantages of using Docker, such as its lightweight and fast start time compared to other related virtualization technology. Next, we derived a taxonomy of 21 major categories representing the purposes of using Docker, including those specific to models such as model management tasks (e.g., testing, training, evaluation), software testing, and managing the different environmental parameters. We believe that other ML engineers can learn about using Docker %\heng{docker vs. Docker}
for the similar purposes in their future deployment of ML software projects. Moreover, we showed that ML engineers use Docker images mostly to help with the platform portability, such as transferring the software across the operating systems, runtimes such as CPU, GPU usage, and language constraints. However, we also found that more resources may be required to run the Docker images for building ML-based software projects due to the large number of files contained in the image layers with deeply nested directories. Finally, we observe that a small set of the contained files occupy relatively large image space, which call for more efficient approaches (e.g., using efficient compression) to store these large files.
%\heng{Finally, we observe that a small set of the contained files occupy relatively large image space, which call for more efficient approaches (e.g., using efficient compression) to store these large files.}
%the ML-based software projects that use Docker into six (6) major groups following manual analysis as the initial steps. We found that the category `Application' is the ML software that mainly uses Docker followed by the MLops categories. Our results indicate that developers adapt Docker in deploying ML-based software projects for production purposes. Indeed this is not surprising given the numerous advantages of using Docker, such as its lightweight and fast start time compared to other related virtualization technology. Moreover, we observed that ML engineers in the ML based repositories related tutorials and documentation. 

%In Figure~\ref{fig:purpose} we reported the 18 major categories representing the purposes for using Docker in the ML-based  software projects. We show that the ML engineers use Docker for different purposes, including those specific to ML models such as model management tasks (e.g., Testing, Training, evaluation), software testing, and managing the different environmental parameters. We believe that other ML engineers can use our summary to learn about the various purposes for using Docker when automating similar tasks.


%In \textbf{RQ3} we were interested in understanding the main functionality that ML engineers use Docker for by analyzing the information within the Dockerfiles such as the executed instructions, the base images used. In Figure~\ref{fig:instructions-composition} we showed that the most used are the RUN instruction due to its generic nature of that allows for the execution of any viable (non-interactive) shell command within the container. For this reason, we further provide the breakdown of the commonly executed instructions into five major categories: Dependencies, Build/ Execution, FileSystem, User permission and Environment settings. Moreover, in Figure~\ref{fig:Docker-category} we showed that the Filesytem and Dependencies related instructions are the most executed across most of the studied ML-based  software projects. Next, we examined the base images and their types for building the images for ML-based  software projects. Our finding indicates that ML engineers use different base images consisting of both official and community-related images. The most used base images are related to the operating system (e.g., ubuntu, debian, centos), platform runtime (e.g., nvidia/cuda), language runtime (e.g., alpine, python, goland, node), and DL frameworks (such as tensorflow/tensorflow, pytorch/ pytorch).

%In the final part of our study, we examined the characteristics of the actual Docker images used in ML-based  software projects. We showed that on the one hand, the images across the ML-based  software projects slightly differ in terms of the configuration file size, the number of layers, and the target hardware architecture (seen in ToolKit category). We invite future research to investigate the reasons for the difference in the Docker images. Moreover, our analysis indicates that different types of files contribute to the larger size of the Docker image layer such as the shared library file, debian file. We recommend that more works can be proposed to minimize the computation overhead during the image layer size.


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> tables/tbl_summary_files.tex <==
\begin{table*}[t]
    \centering
    \tiny
    \caption{The high-level categories of file (file types) compose in the Docker image, their respective size/ capacity in Megabytes (MB) across the studied ML-based software projects and description/ examples of the file type.}
    \label{tab:image-summary}
    %\scalebox{0.75}{
    \begin{adjustbox}{width=\linewidth,center}
    \begin{tabular}{l | c m{2cm} m{2cm} r r r m{8cm}}\toprule
    
  \rowcolor{gray!15}    
 \textbf{File Types}&	\textbf{Model}&\textbf{Application System}&\textbf{MLOps/ AIOps}& \textbf{Toolkit}& \textbf{DL Framwork}& \textbf{Documentation}&\textbf{Descriptions/ Examples}\\\midrule
\textbf{Git}&	367&	358&	560.5&	497.5&	574&	337&Git related files contained in .git folder\\
 \rowcolor{gray!10}
\textbf{Security}&	664.7&	212.2&	0.2&	57.1&	228.9&	236.3&Security related files such as certificates files, keystore, ssh, openssh, ssl, md5, .pem.\\	

\textbf{PEP}&	510.5&	0&	378&	566&	27.9&	57&Files associated with per user site-packages directory where Python packages locally.\\
 \rowcolor{gray!10}
\textbf{Model/ Weights}&	543&	400&	995.7&	25.3&	2.2&	11.6&Models or model weights saved using the popular format e.g., `.pb', `.hdf5', `.pkl', `.mlmodel', `.ckpt', `.onnx'.\\	
 
%\textbf{Video}&	6&	264&	32&	5&	336&	102&Video related files e.g., `.3gp', `.mov', `.mp4', `.m4a', `.m4v', `.mpg', `.wmv', `.avi', `.flv'.\\

\textbf{Image}&	68.2&	22&	1.8&	162&	33&	64.8&images e.g., `.png', `.jpeg', `.svg', `.fits', `.tiff', `.eps', `.gif', `.pic', `.ico', `.jpg', `.xpm', `.pgm'\\
\rowcolor{gray!10}
\textbf{Audio}&	6&	255&	1.6&	1.6&	151.2&	78&Audio files e.g., `.mp3', `.wav', `.aif', `.ogg', `.mid', `.mpa'.\\

\textbf{Web Service}&	526.4&	145&	10.8&	1.9&	13.5&	67& Files associated with the web services e.g., `.asp', `.war', `.cfm', `.cgi', `.apache'\\	
\rowcolor{gray!10}
\textbf{Cached}&	45.3&	1.1&	0&	81&	13.6&	88.8& Cached cached data stored to speed up the performance, usually stored in .cache directory. \\

\textbf{Archival}&	17.5&	39.7&	15.2&	712&	210&0& Archived data e.g., `.zip', `.gzip', `.tar', `.xz', `.bzip', `.bz2'. \\
\rowcolor{gray!10}
\textbf{EOL}&	483&	2.3&	26.7&	59.8&	3&	3.7& Executions, Object code, Library  including the ELF/COFF e.g., `.so', `.o', intermediate compiled, ubuntu, debian, bin \\

\textbf{Script/ Source}&	238&	5&	5.3&	10.3&	13&	0&\\
\rowcolor{gray!10}
\textbf{Documents}&	8&	0&	5.2&	99.1&	4&	381\\

\textbf{Makefile}&	3.4&	1.8&	1.3&	996	&1.8&	3.4& Make related source code (e.g., cmake, `.mk', `qmake', `.pmk', `.make', `cpack', `ctest') containing the descriptions of tools designed to build, test, and package software.\\
\rowcolor{gray!10}
\textbf{Data/Database}&	1.3&	1.2&	1.2&	1.2&	1.2	&1.1& Data files (e.g., csv, json, `.dat', `.npy', `.log') and Database related storage (e.g., `sqlite', `.db', `.dbf', `.mdb', `.pdb') usually used as input or output\\	
%\rowcolor{gray!10}
\textbf{Others}&	220&	41.2&	4.1&	220	&257.6&	0& Uncategoried files \\     
     
\bottomrule
    
    \end{tabular}
    \end{adjustbox}
    %}

\end{table*}
